WaveHoltz: Iterative Solution of the Helmholtz Equation via the Wave Equation

A new idea for iterative solution of the Helmholtz equation is presented. We show that the iteration which we denote WaveHoltz and which filters the solution to the wave equation with harmonic data evolved over one period, corresponds to a coercive operator or a positive definite matrix in the discretized case.

==> multiplefreq.tex <==
%!TEX root = WaveHoltz.tex

\subsection{Multiple Frequencies in One Solve}\label{sec:multifreq}
We can use the WaveHoltz algorithm to solve for multiple frequencies at once. 
Suppose we look for the solutions $u_i$ of
$$
  \nabla\cdot(c^2(x)\nabla u_i) + \omega_i^2u_i = f_i(x),\qquad i=1,\ldots, N,
$$
with the same $c$ and boundary condition for all $i$.
To find those solutions we include all frequencies in the
wave equation part of the iteration (\ref{eq:apa}), and solve
  \begin{align}
%    \pdiff{^2w}{t^2} = c^2(x) \pdiff{^2w}{x^2} 
    w_{tt} = \nabla\cdot (c(x)^2 \nabla w)
    - \sum_{i=1}^N f_i(x)\cos(\omega_i t).
\label{eqn:combined_wave}
  \end{align}
We then seek a decomposition 
\begin{equation}
w(x,t) \equiv \sum_{i=1}^N u_i(x) \cos(\omega_i t), \label{eq:decomp_mul_freq}
\end{equation}
of the solution. The 
filtering part of the
WaveHoltz iteration is also updated to reflect the multiple frequencies 
\begin{align*}
    v_{n+1}  = \frac{2}{T} \int_0^T \left(\sum_{i=1}^N\cos (\omega_i t) - \frac{1}{4} \right) w(x,t) \, dt.
\end{align*}
As before we take $v_0 = 0$ when we deal with energy conserving boundary conditions. To this end we assume that the frequencies are related by an integer multiple in a way so that  the period $T$ can be chosen based on the lowest frequency. 

The different $u_i(x)$ in (\ref{eq:decomp_mul_freq}) can be found as follows. Once we have found the time periodic solution to (\ref{eqn:combined_wave}) evolve one more period and sample $w(x,t)$ at $N$ distinct times $t_j, \, j = 1,\ldots,N$. We then have 
\[
u_i(x) = \sum_{j = 1}^{N} \beta_{ij} w(x,t_j),
\]
where the coefficients $\beta_{ij}$ are the elements of $A^{-1}$ with the elements of $A$ being  $a_{ij} = \cos(\omega_j t_i)$. 


==> period_doubling.tex <==
%!TEX root = WaveHoltz.tex
\subsection{Multiple Frequencies in one Solve}
We can use the WaveHoltz algorithm to solve for multiple frequencies at once. 
\begin{comment}

equation  linearity of the wave equation, we next study how the CG accelerated WaveHoltz iteration converges with respect to the number of frequencies sought. 
Suppose that we are interested in solving a sequence of Helmholtz equations in $1$D (the generalization to multiple dimensions follows immediately):
   \begin{align*}
     c^2(x) \frac{d^2u_i}{dx^2} + \omega_i^2 u_i = f_i(x), \quad i = 1, 2, \dots, N,
   \end{align*}
each with appropriate boundary conditions and frequencies $\omega_i$. We can 
reformulate each of the above problems as a set of wave equations
   \begin{align*}
     \pdiff{^2w_i}{t^2} &= c^2(x) \pdiff{^2w_i}{x^2} - f(x)\cos(\omega_i t), \quad i = 1,2,\dots, N,
   \end{align*}
with appropriate boundary conditions where $w_i(x,t) = u_i(x) \cos(\omega_i t)$
for $i = 1,2,\dots,N$. 
\end{comment}
To do so we solve
  \begin{align*}
    \pdiff{^2w}{t^2} = c^2(x) \pdiff{^2w}{x^2} - \sum_{i=1}^N f_i(x)\cos(\omega_i t), 
\label{eqn:combined_wave}
  \end{align*}
and seek a decomposition 
\begin{equation}
w(x,t) \equiv \sum_{i=1}^N u_i(x) \cos(\omega_i t), \label{eq:decomp_mul_freq}
\end{equation}
of the solution. The WaveHoltz iteration is updated to reflect the multiple frequencies 
\begin{align*}
    v_{n+1}  = \frac{2}{T} \int_0^T \left(\sum_{i=1}^N\cos (\omega_i t) - \frac{1}{4} \right) v_{n}(x,t) \, dt.
\end{align*}
As before we take $v_0 = 0$ when we deal with energy conserving boundary conditions. To this end we assume that the frequencies are related by a integer multiple in a way so that  the period $T$ can be chosen based on the lowest frequency. 

The different $u_i(x)$ in (\ref{eq:decomp_mul_freq}) can be found as follows. Once we have found the time periodic solution to (\ref{eqn:combined_wave}) evolve one more period and sample $w(x,t)$ at $N$ distinct times $t_j, \, j = 1,\ldots,N$. We then have 
\[
u_i(x) = \sum_{j = 1}^{N} \beta_{ij} w(x,t_j),
\]
where the coefficients $\beta_{ij}$ are the elements of $A^{-1}$ with the elements of $A$ being  $a_{ij} = \cos(\omega_j t_i)$. 

\begin{comment}
The $u_i(x)$ are then fond as the linear combinations  and solve the $N \times N$ linear system of equations $A {
\bf u} = {\bf w}$ where the elements of $d$       

If the iteration converges 
after $M$ iterations, then we have that the solution $v_M$ at the end of the 
iteration is a linear combination of Helmholtz solutions as follows:  

  \begin{align} 
    v_{M} (x,t) = \sum_{i=1}^N u_i(x) \cos(\omega_i t) \label{eqn::MultFreqSol}.
  \end{align}
Let $x$ be fixed and consider $N$ time points $t_j \in [0,T]$. Evaluation of 
\eqref{eqn::MultFreqSol} at time points $t_j$ gives the system of equations
  \begin{align*}
    v_M(x,t_j) = \sum_{i=1}^N u_i(x) \cos(\omega_i t_j), \quad j = 1, 2, \dots, N,
  \end{align*}
which may be written as the matrix system
  \begin{align}
    \begin{bmatrix}
      \cos(\omega_1 t_1) & \cos(\omega_2 t_1) & \cdots & \cos(\omega_N t_1) \\
      \cos(\omega_1 t_2) & \cos(\omega_2 t_2) & \cdots & \cos(\omega_N t_2) \\ 
      \vdots & \vdots & \ddots & \vdots\\ 
      \cos(\omega_1 t_N) & \cos(\omega_2 t_N) & \cdots & \cos(\omega_N t_N)
    \end{bmatrix}
    \begin{bmatrix}
      u_1(x) \\ u_2(x) \\ \vdots \\ u_N(x)
    \end{bmatrix}
    = 
    \begin{bmatrix}
      v_M(x,t_1) \\ v_M(x,t_2) \\ \vdots \\ v_M(x,t_N)
    \end{bmatrix}. \label{eqn::MatrixMultFreq}
  \end{align}

It follows from the above matrix that the evolution of the converged solution $v_M$ 
forward in time to the time points $t_j$ yields a matrix system that is solvable for 
each individual frequency solution $u_i$, i.e. it is possible to recover multiple 
Helmholtz solutions from a single converged iterate at the small cost of an additional 
forward wave solve to the time points $t_j$. 

As a simple example, consider the case where $N=2$ and $\omega_2 = 2 \omega_1 = 2 \omega$ with the 
forcing $f(x)(\cos(\omega_0 t) + \cos(\omega_1 t))$. Then, when we have converged we can use the fact 
that at a half-period we have $\cos(  \frac{\omega_0T}{2} ) = -1 $ while 
$\cos( \frac{\omega_1 T}{2} ) = 1$. Thus, by two linear combinations of the double forced solution 
at times $t=0$ and $t = T/2$ we can extract both $u_0(x)$ and $u_1(x)$ at the same cost as solving 
for $u_0$ alone. In the general case \eqref{eqn::MatrixMultFreq} care should be taken to ensure that 
the left hand matrix $A_{ij} = \cos(\omega_i t_j)$ is not singular to successfully 
recover each frequency solution.
\end{comment}

As an illustration we set $\omega = 1$ and $\omega_j = 2^{j-1} \omega$ for $j = 1,\ldots,4$ 


%and find the solutions $u_j(x) = \sin(\pi x)/(\omega_j^2 - \pi^2)$ resulting from the forcing $f_j(x) = \sin(\pi x)$.
%To illustrate this concept, let $\omega >0$ be fixed and consider the family of $1$D Helmholtz problems $d^2u_j/dx^2 + \omega^2_j u_j = f_j(x)$ with Dirichlet boundary conditions where $x \in [0,1]$ and $\omega_j = 2^{j-1} \omega$. In this first example, we let 

\begin{comment}
We use an equispaced grid $x_i = ih$ for $i = 1,2,\dots, D$ where $h = 1/(D+1)$. 
In the following examples, we let $D = 100$ (a fairly coarse grid, should this be made larger?) 
and use a fourth order finite difference approximation for the Laplacian and the five-stage, 
fourth order strong stability preserving method of Spiteru and Ruuth (SSPRK54) in time. 
We use a Gaussian quadrature rule to compute the integral operator, with a third order Hermite 
polynomial interpolation to evaluate at the Gauss nodes in time. We examine the case where we 
include $10$ terms in \eqref{eqn:combined_wave} for frequencies $\omega, 2\omega, 4\omega, 
\dots, 2^9\omega$ where $\omega = 1.22$.
\begin{table}[H]
  \centering
  \resizebox{0.75\columnwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|c|}
  \hline
  & $10$ & $50$ & $100$ & $200$ & $500$ & $1000$ & $5000$ \tabularnewline
  \hline
  $\omega$ & 1.53e+1 & 2.61e-2 & 1.33e-2 &7.86e-3 &7.38e-3 &2.76e-6 & 8.76e-9 \tabularnewline
  \hline
  $2\omega$ & 5.62e-1 & 9.60e-2 & 4.90e-3 & 2.89e-2 &2.71e-2 &1.02e-5 & 1.81e-8 \tabularnewline
  \hline
  $4\omega$ & 1.57 & 2.68e-1 & 1.37e-2 & 8.08e-2 & 7.58e-2 & 2.85e-5 &2.31e-9 \tabularnewline
  \hline 
  $8\omega$ & 9.75 & 1.67e-1 & 8.51e-3 & 5.01e-2 & 4.70e-2 & 1.77e-5 & 1.84e-8\tabularnewline
  \hline 
  $16\omega$ & 8.70 & 1.49 & 7.59e-2 & 4.47e-1 & 4.19e-1 & 1.58e-4 & 3.35e-8\tabularnewline
  \hline 
  $32\omega$ & 6.41 & 1.10 & 5.59e-2 & 3.29e-1 & 3.09e-1 & 1.16e-4 & 2.45e-7\tabularnewline
  \hline 
  $64\omega$ & 4.09e+2 & 6.99e+2 & 3.57 & 2.10e+1 &1.97e+1 & 7.42e-3 & 4.97e-7 \tabularnewline
  \hline 
  $128\omega$ & 2.12e+2 & 3.62e+1 & 1.85e-1 & 1.09 & 1.02 & 3.87e-4 & 3.16e-6 \tabularnewline
  \hline  
  $256\omega$ &  3.02e+4 & 5.17e+3 & 2.64e+2 & 1.55e+3 & 1.46e+3 & 5.48e-1 & 4.76e-5 \tabularnewline
  \hline 
  $512\omega$ &  1.61e+4 & 2.75e+3 & 1.40e+2 & 8.27e+2 & 7.58e+2 & 2.91e-1 & 3.05e-4 \tabularnewline
  \hline 
  \end{tabular}}
  \caption[]
  {\small Relative $L_2$ errors for the period doubling problem. From left to right 
  the number of Gauss quadrature nodes is increased. From top to bottom the relative 
  error to the true solution for increasing frequencies is shown. } 
\end{table}
We see from the above table that in order to capture increasingly larger frequencies 
it is necessary to increase the number of quadrature nodes used. Unsurpringly, the error 
of higher frequency solutions is larger than that of the base frequency $\omega$.
\end{comment}

We again consider the same domain as above with a standard second order difference in 
both space and time (the same discretization as in the discrete analysis presented 
earlier) with a point forcing of $f(x) = f_j(x) = -\delta(x-1/2)/h$ for $j= 1, \dots, 4$
and spatial step $h$. The filtering operator is evaluated with trapezoidal rule 
in this case and the base frequency is $\omega = 1$. We examine the convergence 
with decreasing $h$ in Figure \ref{fig:1d_delta_multiple_freq} below.
\begin{figure}[H]
	\graphicspath{{figures/}}
	\begin{center}
	\includegraphics[width=0.5\textwidth]{1D_secondOrderSpatial_errorDelta.eps}
	\caption{Convergence of the solution for the CG accelerated  WaveHoltz 
	iteration with a point forcing.
	\label{fig:1d_delta_multiple_freq}}
	\end{center}
\end{figure}
From Figure \ref{fig:1d_delta_multiple_freq} it can be seen that each frequency
has second order convergence.
